From Language to Locomotion: Retargeting-free Humanoid Control via Motion Latent Guidance

Natural language offers a natural interface for humanoid robots, but existing language-guided humanoid locomotion pipelines remain cumbersome and untrustworthy. They typically decode human motion, retarget it to robot morphology, and then track it with a physics-based controller. However, this multi-stage process is prone to cumulative errors, introduces high latency, and yields weak coupling between semantics and control. These limitations call for a more direct pathway from language to action, one that eliminates fragile intermediate stages. Therefore, we present RoboGhost, a retargeting-free framework that directly conditions humanoid policies on language-grounded motion latents. By bypassing explicit motion decoding and retargeting, RoboGhost enables a diffusion-based policy to denoise executable actions directly from noise, preserving semantic intent and supporting fast, reactive control. A hybrid causal transformer-diffusion motion generator further ensures long-horizon consistency while maintaining stability and diversity, yielding rich latent representations for precise humanoid behavior. Extensive experiments demonstrate that RoboGhost substantially reduces deployment latency, improves success rates and tracking precision, and produces smooth, semantically aligned locomotion on real humanoids. Beyond text, the framework naturally extends to other modalities such as images, audio, and music, providing a universal foundation for vision-language-action humanoid systems.

==> sections/01_introduction.tex <==
\section{Introduction}
% Natural language is the most intuitive interface humans have ever known. When we say “run to the door and turn around before you stop,” we convey not just a sequence of motions, but an intent shaped by years of embodied experience—anticipating friction, balance, momentum, and spatial constraints. For humanoid robots to become truly accessible partners in everyday environments, they must go beyond literal interpretation and develop a similar understanding: one that unifies linguistic semantics with physical dynamics. 

% Recent advances in text-to-motion (T2M) generation have brought us closer to this goal. Powered by large language models and diffusion architectures, existing motion generators can synthesize rich, diverse human motion from free-form text~\citep{li2024lamp, chen2023executing, guo2024momask, li2024mulsmo, tevet2022human}. These models encode vast priors about how people move, offering a compelling blueprint for robot behavior. However, a critical gap remains: these systems understand what to do, but not how to do it under physical laws. They operate in kinematic space, blind to inertia, contact forces, or joint limits—producing motions that may look plausible in simulation, yet fail catastrophically on robot. 

% Prior works~\citep{yue2025rl, serifi2024robot, shao2025langwbc} attempt to bridge this gap through such a hierarchical generation-execution pipeline: \textbf{(i)} a latent motion representation is synthesized from natural language, \textbf{(ii)} decoded into a semantically consistent human motion, \textbf{(iii)} retargeted to the robot’s kinematic structure, and \textbf{(iv)} tracked in simulation or on hardware via a physics-based controller~\citep{peng2018deepmimic, ji2024exbody2, chen2025gmt, he2025asap}. 

% While effective on well-behaved trajectories, this intuitively appealing and widely adopted pipeline reveals three fundamental limitations. First, information degradation accumulates across stages. The generated motion is inherently noisy and imperfect due to the limitations of current motion generators. However, existing frameworks deploy these motions as is, making real-world performance critically dependent on the generator's fidelity. Furthermore, the retargeting process—often based on kinematic heuristics or optimization—introduces additional distortions, particularly when adapting human motions to morphologically distinct robots. These cascading errors erode both dynamic feasibility and semantic integrity.  Second, the inference pipeline is prohibitively sequential and slow. Execution requires traversing multiple non-differentiable stages: text-conditioned latent generation, motion decoding, robot-specific retargeting, and finally, controller deployment. This rigid cascade cannot react in real time and imposes significant latency, limiting its applicability in interactive or time-sensitive scenarios. Finally, the architecture of motion generators themselves remains suboptimal. Dominant approaches fall into two categories: autoregressive models over discrete tokens and diffusion-based continuous generative models. The former suffers from quantization-induced information loss and limited long-horizon coherence, while the latter often lacks explicit temporal structure and struggles with fine-grained semantic alignment. 

% Although recent efforts~\citep{yue2025rl} incorporate semantic alignment for refinement, gradients rarely propagate directly into the generator; instead, tuning often primarily affects the decoder, with limited impact on the motion generator, potentially leaving the generative prior under-optimized.  As a result, the system learns to “patch” outputs rather than truly understand the relationship between language and physical action.  Together, these issues expose a deeper flaw: the entire pipeline operates under an illusion of comprehension—one that mistakes surface-level motion synthesis for embodied understanding. To bridge these gaps, we argue for a paradigm shift in how generative models interface with control systems. Rather than treating the motion generator as a black-box artist producing trajectories to be later adapted and tracked, we propose to leverage its rich, semantically grounded latent representations as direct conditioning signals for policy learning. 

% In this work, we propose XXX, a novel retargeting-free, latent-driven language-guided humanoid locomotion framework that unifies text-to-motion with end-to-end action synthesis. Instead of decoding and retargeting full-body human motions, our policy uses the motion generator’s latent representation—enriched by LaMP~\citep{li2024lamp}—as a semantic anchor to guide a diffusion-based policy in denoising robot actions directly from noise. This implicit coupling eliminates multiple error-prone stages, reduces deployment latency, and preserves fine-grained intent throughout execution. Furthermore, to combine the strengths of autoregressive modeling and diffusion priors, we adopt a hybrid transformer-diffusion architecture: the transformer captures long-range temporal structure and semantic coherence, while the diffusion model ensures diverse and stable motion sequences.

% Our approach overturns the prevailing paradigm by introducing latent-driven humanoid locomotion control, yielding a more streamlined and coherent pipeline while significantly reducing noise accumulation across stages. Furthermore, we present the first diffusion-based humanoid policy, which enables smooth and natural motion generation, with accelerated sampling via DDIM~\citep{song2020denoising} for real-time deployment. 

Natural language is the most intuitive interface humans have ever known, yet translating free-form instructions into physically feasible humanoid motion remains challenging. 
Recent text-to-motion (T2M) models can synthesize rich, diverse human motion from free-form text~\citep{li2024lamp, chen2023executing, guo2024momask, li2024mulsmo, tevet2022human}, encoding vast priors about “what” to do. 
However, they operate primarily in kinematic space—blind to inertia, contact forces, and joint limits—so motions that appear plausible in animation often fail on real robots. 
To make humanoids truly accessible partners, we must bridge linguistic semantics and physical dynamics, not just imitate human pose sequences.

Prior works~\citep{yue2025rl, serifi2024robot, shao2025langwbc} typically follow a hierarchical generation–execution pipeline: \textbf{(i)} synthesize a latent from language, \textbf{(ii)} decode a human motion, \textbf{(iii)} retarget to the robot’s kinematics, and \textbf{(iv)} track via a physics-based controller~\citep{peng2018deepmimic, ji2024exbody2, chen2025gmt, he2025asap}. While effective on well-behaved trajectories, this paradigm faces three systemic limitations. First, errors accumulate across decoding, retargeting, and tracking. Noisy motion generation and morphology mismatch introduce distortions that undermine both feasibility and semantics. Second, the pipeline is sequential and slow. Multiple stages incur latency and hinder real-time interaction. Third, modeling gaps persist. Autoregressive approaches suffer quantization and long-horizon drift; diffusion models lack explicit temporal structure and fine-grained alignment.

Recent refinements~\citep{yue2025rl} add semantic alignment, but gradients seldom shape the motion generator itself; most tuning targets the decoder, leaving the generative prior under-optimized. In practice, the system “patches” outputs instead of learning a tight coupling between language and control. We argue for a simpler interface: use semantically grounded motion latents directly as conditioning signals for control policies, avoiding fragile decoding and retargeting altogether.

To address these issues, we propose GhostBot, a retargeting-free, latent-driven framework that unifies text-to-motion with end-to-end humanoid action synthesis. Rather than decoding and retargeting full-body human motion, GhostBot leverages LaMP-enhanced motion generated latents as semantic anchors to condition a diffusion-based humanoid policy that denoises humanoid actions directly from noise. This implicit coupling removes error-prone stages, preserves fine-grained intent, and enables fast, reactive control. To balance long-range temporal coherence and robust motion synthesis, GhostBot employs a causal autoencoder combined with a hybrid transformer–diffusion architecture in the motion generation stage. This design integrates the strengths of autoregressive modeling and continuous latent encoding: it mitigates information loss induced by discrete tokenization while enhancing the diversity of generated latents — thereby providing downstream policies with richer, more expressive semantic conditioning for precise control. During policy training, the pretrained motion generator is kept frozen or lightly finetuned to preserve semantics and produce implicit representations for the downstream policy — entirely bypassing explicit human pose decoding. The policy, in turn, learns to generate physically executable actions directly from noise, conditioned on these latent representations.

Our approach overturns the prevailing pipeline by directly coupling language-grounded motion latents with physics-based control, substantially reducing noise accumulation and deployment delay. We further present, to our knowledge, the first diffusion-based humanoid policy for language-guided locomotion, achieving smooth and natural motion with accelerated sampling via DDIM~\citep{song2020denoising} for real-time deployment. This design affords three practical benefits. First, a retargeting-free paradigm avoids the information loss and time cost incurred by motion retargeting, improving tracking performance while substantially reducing end-to-end latency. Second, latent-driven action synthesis enables the policy to optimize directly against the motion generator, bypassing the decoder and preventing real-world failures caused by low-quality explicitly generated motions. Finally, conditioning on latent representations preserves strong semantic alignment, allowing the robot to reliably follow fine-grained instructions (e.g., left-right and clockwise-counterclockwise).


In summary, our key contributions can be summarized as follows:
\begin{itemize}
\item We propose GhostBot, a retargeting-free and latent-driven framework for language-guided humanoid locomotion, which eliminates error-prone decoding and retargeting stages by directly leveraging semantic-rich motion latents for end-to-end policy learning.

\item We introduce the first diffusion-based humanoid policy that denoises robot actions from noise guided by text-conditioned motion latents, enabling smooth, diverse, and physically plausible motion generation with DDIM-accelerated sampling for real-time deployment.

\item We present a hybrid transformer-diffusion architecture that combines the long-range temporal coherence of autoregressive modeling with the stochastic stability of diffusion models in humanoid, achieving high-fidelity motion synthesis and language-motion alignment.

\item Through extensive experiments, we demonstrate the effectiveness, simplicity, and generality of our approach, successfully enabling text-guided real-world humanoid locomotion control.
\end{itemize}
